Zero modes of quantum graph Laplacians and an index theorem

We study zero modes of Laplacians on compact and non-compact metric graphs with general self-adjoint vertex conditions. In the first part of the paper the number of zero modes is expressed in terms of the trace of a unitary matrix $\mathfrak{S}$ that encodes the vertex conditions imposed on functions in the domain of the Laplacian. In the second part a Dirac operator is defined whose square is related to the Laplacian. In order to accommodate Laplacians with negative eigenvalues it is necessary to define the Dirac operator on a suitable Kre\u{\i}n space. We demonstrate that an arbitrary, self-adjoint quantum graph Laplacian admits a factorisation into momentum-like operators in a Kre\u{\i}n-space setting. As a consequence, we establish an index theorem for the associated Dirac operator and prove that the zero-mode contribution in the trace formula for the Laplacian can be expressed in terms of the index of the Dirac operator.

==> def.tex <==
%
\newcommand{\mfS}{\mathfrak{S}}
\newcommand{\wh}{\widehat}
\newcommand{\dz}{d}
\newcommand{\Je}{J_{\mc{E}}}
\newcommand{\bva}{\kz^{\mc{V}}}
\newcommand{\Lt}{L^2\lk\Lambda^0\Gamma\rk}
\newcommand{\Psy}{P_{\sy}}
\newcommand{\Pasy}{P_{\asy}}
\newcommand{\ex}{\mathrm{ex}}
\newcommand{\inte}{\mathrm{int}}
\newcommand{\new}{\mathrm{new}}
\newcommand{\sy}{\mathrm{sy}}
\newcommand{\asy}{\mathrm{asy}}
\newcommand{\init}{\mathrm{in}}
\newcommand{\eb}{\eref}
\newcommand{\Pbse}{Q^{\bot}}
\newcommand{\Pb}{Q}
\newcommand{\ord}{\mathrm{ord}}
%
\newcommand{\bal}{\bsy{\alpha}}
\newcommand{\bbe}{\bsy{\beta}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\wbz}{\widetilde{\bz}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\va}{\boldsymbol{a}}
\newcommand{\bn}{\boldsymbol{0}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\Sk}{\mfS(k;A,B)}
\newcommand{\Tk}{T_{\mc{E}}(k;\bsy{l})}
\newcommand{\FKW}{\mh{FKW}}
\newcommand{\Po}{\mh{P}}
%
\newcommand{\Ind}{\mathrm{Ind}}
\newcommand{\Mat}{\mathrm{Mat}}
\newcommand{\ind}{\mathrm{ind}}
\newcommand{\im}{\mathrm{Im}}
\newcommand{\ran}{\mathrm{ran}}
\newcommand{\re}{\mathrm{Re}}
\newcommand{\term}{\mathrm{term}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\Or}{\mathrm{Or}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\ui}{\mathrm{i}}
\newcommand{\ue}{\mathrm{e}}
\newcommand{\gz}{{\mathbb Z}}
\newcommand{\rz}{{\mathbb R}}
\newcommand{\nz}{{\mathbb N}}
\newcommand{\kz}{{\mathbb C}}
\newcommand{\qz}{{\mathbb Q}}
\newcommand{\lek}{\left[}
\newcommand{\rek}{\right]}
\newcommand{\rw}{\right>}
\newcommand{\lb}{\left\|}
\newcommand{\rb}{\right\|}
\newcommand{\lw}{\left<}
\newcommand{\eins}{\mathds{1}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\hata}{\widehat}
\newcommand{\lk}{\left(}
\newcommand{\rk}{\right)}
\newcommand{\lgk}{\left\{}
\newcommand{\rgk}{\right\}}
\newcommand{\mf}{\mathfrak}
\newcommand{\mc}{\mathcal}
\newcommand{\ba}{\begin{aligned}}
\newcommand{\ea}{\end{aligned}}
\newcommand{\eq}{\eqalign}
\newcommand{\wt}{\widetilde}
\newcommand{\mh}{\mathrm}
\newcommand{\lin}{\mathrm{lin}}
\newcommand{\bsy}{\boldsymbol}
\newcommand{\bma}{\left(
\begin{array}
}
\newcommand{\ema}{\end{array}
\right)}
%
\newtheorem{theoremd}{Theorem and Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{defn}{Definition}
\newtheorem{rem}{Remark}
\newtheorem{exa}{Example}


